Best Friends Forever (BFF): Finding Lasting Dense Subgraphs

Graphs form a natural model for relationships and interactions between entities, for example, between people in social and cooperation networks, servers in computer networks, or tags and words in documents and tweets. But, which of these relationships or interactions are the most lasting ones? In this paper, we study the following problem: given a set of graph snapshots, which may correspond to the state of an evolving graph at different time instances, identify the set of nodes that are the most densely connected in all snapshots. We call this problem the Best Friends For Ever (BFF) problem. We provide definitions for density over multiple graph snapshots, that capture different semantics of connectedness over time, and we study the corresponding variants of the BFF problem. We then look at the On-Off BFF (O^2BFF) problem that relaxes the requirement of nodes being connected in all snapshots, and asks for the densest set of nodes in at least $k$ of a given set of graph snapshots. We show that this problem is NP-complete for all definitions of density, and we propose a set of efficient algorithms. Finally, we present experiments with synthetic and real datasets that show both the efficiency of our algorithms and the usefulness of the BFF and the O^2BFF problems.

==> proofs.tex <==
Due to lack of space, we only give a sketch of the proof. The intuition behind the proof is that if there is a dense set of nodes $A$ in the graph history that maximizes the density, if the nodes of the set have low degree in a single snapshot, the {\algobffmm} will remove nodes from the set, and thus never return it as a candidate solution.

For the {\problemam} problem we construct a counter-example where the graph sequence is composed of graphs that consist of a set $A$ of $n$ nodes that form a clique, and a single edge. In the last snapshot the nodes in the set $A$ are disconnected. The {\algobffmm} will iteratively remove these nodes, and thus always yield candidate solutions $S_i$ with $f_{am}(S_i) = 1$, while the optimal solution is $A$ with $f_{ma}(A) = O(n)$.

For the {\problemma} problem we construct a counter-example where the graph sequence is composed of $m$ graphs that consist of a set $A$ of $m$ nodes that form a clique, and a set $B$ of $m^2$ nodes that form a cycle. In the last snapshot the nodes in the set $A$ are disconnected. The {\algobffmm} will iteratively remove the nodes in $A$, and thus always yield candidate solutions $S_i$ with $f_{am}(S_i) = \Theta(1)$, while the optimal solution is $A$ with $f_{am}(A) = \Theta(m) = \Theta(\sqrt{n})$.

